Learning Keypoints for Robotic Cloth Manipulation using Synthetic Data

Assistive robots should be able to wash, fold or iron clothes. However, due to the variety, deformability and self-occlusions of clothes, creating robot systems for cloth manipulation is challenging. Synthetic data is a promising direction to improve generalization, but the sim-to-real gap limits its effectiveness. To advance the use of synthetic data for cloth manipulation tasks such as robotic folding, we present a synthetic data pipeline to train keypoint detectors for almost-flattened cloth items. To evaluate its performance, we have also collected a real-world dataset. We train detectors for both T-shirts, towels and shorts and obtain an average precision of 64% and an average keypoint distance of 18 pixels. Fine-tuning on real-world data improves performance to 74% mAP and an average distance of only 9 pixels. Furthermore, we describe failure modes of the keypoint detectors and compare different approaches to obtain cloth meshes and materials. We also quantify the remaining sim-to-real gap and argue that further improvements to the fidelity of cloth assets will be required to further reduce this gap. The code, dataset and trained models are available

==> appendices.tex <==
\appendices
\section{Dataset Details}
Appendix one text goes here.
\section{Keypoint Detector Details}
Appendix two text goes here.
\section{ProcGent Details}
Randomization ranges etc. 

\section{Engineering Findings}

A few things I would like to write down for myself. Probably don't belong in the paper.

Recipe for Sim2real? it is often manual trial and error (e.g. https://developer.nvidia.com/blog/closing-the-sim2real-gap-with-nvidia-isaac-sim-and-nvidia-isaac-replicator/), but still there are some guidelines to follow maybe and some metrics to watch? 



Architecture of a synthetic data generation pipeline:
how to manage the randomization parameters and the diverse 'options' for different aspects of the pipeline.
